RealGUINoise: An Interactive Cross-Platform Benchmark for GUI Agent Robustness under Real-World Interface Noise

Graphical User Interface (GUI) agents and Computer-Using Agents (CUAs) are rapidly becoming practical tools. However, real-world deployment increasingly exposes performance failures and safety risks, while a major yet underexplored source of these problems lies in the complex and noisy conditions of everyday interfaces. Existing benchmarks largely assume clean environments or focus narrowly on security-specific settings, and lack a unified framework for consistent, automated end-to-end evaluation across diverse agents and platforms. Hence, we introduce RealGUINoise, an interactive cross-platform, extensible benchmark for systematically evaluating GUI Agents under common realistic interface noise in fully interactive environments. Specifically, RealGUINoise comprises 42 noise types spanning web, desktop, and mobile tasks and integrates 7 representative agent frameworks. It evaluates these agents on real-world daily tasks through real-time interaction, comparing their performance against task-specific golden rubrics and clean-environment trajectories in terms of reliability, safety, and trajectory-level behavior. Our experiments show that these noises not only degrade task performance but also substantially redirect agents' action trajectories and increase their propensity for unsafe behavior. These findings expose a critical gap between capability in clean environments and dependable operation in real-world settings, establishing RealGUINoise as a testbed for developing more robust and trustworthy GUI agents.

==> Figures/task_distribution.tex <==
\begin{figure}[t]
\centering
\resizebox{\columnwidth}{!}{
\begin{tikzpicture}
\begin{axis}[
    xbar,
    width=0.9\linewidth,
    height=16cm,
    bar width=6pt,
    xlabel={Number of Tasks},
    symbolic y coords={
        BreezyWeather, FindNearBy, NewPipe, ShoppingApp, Transportr,
        Trip, Zhihu, Quora, Temu, {Google Form}, {Movie Download Chinese},
        {HKGolden Forum}, {Google News}, {The New York Times}, CNN, Yandex,
        Wikipedia, Bilibili, Google, Baidu, YouTube, Amazon, BBC
    },
    ytick={
        BreezyWeather, FindNearBy, NewPipe, ShoppingApp, Transportr,
        Trip, Zhihu, Quora, Temu, {Google Form}, {Movie Download Chinese},
        {HKGolden Forum}, {Google News}, {The New York Times}, CNN, Yandex,
        Wikipedia, Bilibili, Google, Baidu, YouTube, Amazon, BBC
    },
    yticklabel style={font=\small},
    xtick style={draw=none},
    axis lines*=left,
    enlarge y limits=0.03,
    nodes near coords,
    every node near coord/.append style={font=\scriptsize},
    xmin=0, xmax=22,
    legend image code/.code={
        \draw[#1] (0cm,-0.1cm) rectangle (0.3cm,0.1cm);
    },
    legend style={
        at={(0.97,0.03)},
        anchor=south east,
        font=\small,
        draw=none
    },
]

\addplot[fill=blue!60!black!70, draw=none, bar shift=0pt] coordinates {
    (1,Trip) (5,Zhihu) (5,Quora) (6,Temu) (6,{Google Form})
    (6,{Movie Download Chinese}) (6,{HKGolden Forum}) (7,{Google News})
    (10,{The New York Times}) (11,CNN) (11,Yandex) (11,Wikipedia)
    (11,Bilibili) (13,Google) (14,Baidu) (14,YouTube) (16,Amazon) (19,BBC)
};
\addlegendentry{Website}

\addplot[fill=orange!80!red!70, draw=none, bar shift=0pt] coordinates {
    (7,BreezyWeather) (7,FindNearBy) (7,NewPipe) (7,ShoppingApp) (7,Transportr)
};
\addlegendentry{App}

\end{axis}
\end{tikzpicture}
}
\caption{Task distribution across websites and mobile apps.}
\label{fig:task-distribution}
\end{figure}

==> Sections/2_Background.tex <==
%%INFO: owner=___ | last-edit=2026-07-13 | final=no
%%TODO: add citations
%%TODO: 2.3+2.4 overlap -- candidate cut if over the 7-page budget
\section{Background}
\label{sec:bg}

\subsection{GUI Agents}
GUI agents are autonomous systems that execute user instructions by interacting directly with graphical user interfaces rather than through task-specific APIs. In our setting, this definition includes both \textbf{desktop/web} environments and \textbf{mobile} environments: a GUI agent may search the web, browse news pages, shop on e-commerce sites, fill forms, or operate smartphone applications through the same high-level instruction-following loop. This cross-platform perspective is important because many real user tasks are not confined to a single software substrate, and practical automation increasingly requires agents that can act across heterogeneous interfaces.

Recent progress in large language models (LLMs) and multimodal large language models (MLLMs) has made such agents substantially more capable. By combining visual perception, language understanding, planning, and action generation, modern GUI agents can interpret screenshots, reason over interface state, and iteratively execute actions such as clicking, typing, scrolling, navigating, and invoking tools. Compared with earlier rule-based or API-driven systems, these agents require much less manual task engineering; compared with demonstration-only systems, they offer more flexible zero-shot or few-shot generalization across tasks and interfaces. As a result, GUI agents are emerging as a general paradigm for interface-level automation on both PCs and smartphones.

\subsection{Perception--Reasoning--Action Loop}
Modern GUI agents are typically built around a closed-loop \emph{perception--reasoning--action} architecture. The \textbf{perception} module gathers observations from the environment, commonly in the form of screenshots, accessibility trees, OCR-extracted text, DOM-like browser structure, or other interface metadata. The \textbf{reasoning} module maintains task context, interprets the current state, decomposes the user objective into intermediate subgoals, and decides what to do next. The \textbf{action} module then executes low-level operations in the environment, such as mouse clicks, keyboard input, touch gestures, scrolling, or tool invocations.

This loop distinguishes GUI agents from standard single-turn language systems. Instead of producing one answer from a fixed input, a GUI agent must repeatedly observe a changing environment, update its internal state, and choose the next action under partial observability. This interactive setting is especially important for both web and mobile tasks, where success depends not only on semantic understanding of the instruction, but also on accurate state tracking, recovery from errors, and adaptation to dynamic interface changes. In practice, even seemingly simple tasks often require long-horizon execution over multiple dependent interface states.

\subsection{Current Evaluation Practice}
The standard way to evaluate GUI agents is to benchmark them on task-oriented environments and report task success or related trajectory-quality metrics. Existing benchmarks have played an important role in advancing the field by measuring skills such as navigation, information retrieval, form completion, and multi-step interaction. In both desktop/web and mobile settings, the dominant evaluation paradigm is to place agents in relatively clean, curated environments and assess whether they can complete the intended objective within a limited interaction budget.

This evaluation paradigm works well for establishing basic agent competence. It is useful for measuring whether an agent can understand instructions, ground interface elements, and execute multi-step plans under controlled conditions. It has also enabled meaningful comparisons across model families and agent frameworks. However, most current evaluations remain either platform-specific, clean by design, or centered primarily on task completion rather than robustness. As a result, they provide only a partial picture of how GUI agents behave outside idealized settings.

\subsection{Robustness Gap in Real Interfaces}
The main limitation of current evaluation practice is that it under-represents the kinds of interface disturbances that dominate real deployment. In realistic web pages and mobile apps, agents must operate under visual clutter, dynamic loading, overlays, pop-ups, deceptive widgets, permission prompts, focus changes, misleading labels, and other forms of interaction noise. These perturbations affect not only perception, but also action selection, trajectory coherence, and safety. A small change in layout or behavior can redirect an agent to the wrong interface element, trigger an unintended side effect, or waste a large fraction of the available interaction budget.

This gap is particularly consequential for cross-platform agents. Web and mobile interfaces differ in layout density, event handling, navigation patterns, and affordances, but both exhibit similar robustness challenges: asynchronous content updates, interface interruptions, ambiguous controls, and context-dependent rendering. Evaluating only in clean desktop pages or only in curated mobile tasks therefore risks overstating deployment readiness. In practice, an agent that performs well in a clean benchmark may still fail once ads, banners, hover interactions, fake search bars, cookie dialogs, autoplay media, or mobile interruptions are introduced.

From a benchmarking perspective, current practice has three concrete limitations. First, it often assumes clean or weakly perturbed interfaces, leaving realistic noise underexplored. Second, evaluation is frequently fragmented across desktop/web and mobile settings, despite the fact that both fall under the broader GUI-agent problem. Third, most existing metrics emphasize task success alone and do not fully capture robustness-related failure modes such as unsafe actions, trajectory degradation, or deviations from clean execution. These limitations motivate a benchmark that treats robustness as a first-class evaluation target rather than as an incidental error source.

\subsection{{\methodname} in Context}
\methodname is designed to address this evaluation gap. Our central premise is that robustness for GUI agents should be measured in \emph{executable}, \emph{cross-platform}, and \emph{noise-aware} environments. To this end, \methodname covers both desktop/web and mobile settings under a unified GUI-agent definition, and organizes realistic perturbations into structured noise categories that can be systematically injected and evaluated. Instead of restricting evaluation to clean interfaces, \methodname measures how agent behavior changes when the environment contains realistic disturbances that affect perception, reasoning, and action.

This design shifts the focus of evaluation from ``can the agent solve the clean task?'' to the more deployment-relevant question: ``can the agent solve the task reliably under realistic interface noise?'' The remainder of the paper follows this perspective. We first define the perturbation taxonomy and benchmark construction process, then describe the executable environments and unified evaluation framework, and finally benchmark representative desktop and mobile agents to characterize the robustness gap of current GUI-agent systems.
